Who Speaks for Ethics? How Demographics Shape Ethical Advocacy in Software Development

The integration of ethics into software development faces significant challenges due to market fundamentalism in organizational practices, where profit often takes precedence over ethical considerations. Additionally, the critical influence of practitioners' individual backgrounds on ethical decision-making remains underexplored, highlighting a gap in comprehensive research. This is especially essential to understand due to the demographic imbalance in software roles. This study investigates ethical concerns in software development, focusing on how they are perceived, prioritized, and addressed by demographically different practitioners. By surveying 217 software practitioners across diverse roles, industries, and countries, we identify critical barriers to ethical integration and examine practitioners' capacity to mitigate these issues. Our findings reveal pronounced demographic disparities, with marginalized groups - including women, BIPOC, and disabled individuals - reporting ethical concerns at higher frequencies. Notably, marginalized practitioners demonstrated heightened sensitivity to ethical implementation and greater empowerment to address them. However, practitioners overall often lack the support needed to address ethical challenges effectively. These insights underscore the urgent need for reforms in software education and development processes that center on diverse perspectives. Such reforms are essential to advancing ethical integration in software development and ensuring responsible computing practices in an increasingly complex technological landscape.

==> leftovers.tex <==

%Finally, for the time practitioners spend testing with end-users before releasing features \textbf{(RQ2.8)}, 35.26\% (61/173) indicated weeks, while 49.13\% (85/173) reported months. 



% \fbox{\begin{minipage}{.9\linewidth}\textbf{Answer to RQ2:} The  software development process can facilitate ethical concerns. While ethical issues are emphasized during onboarding, organizational factors like deadlines and investor expectations often interfere with addressing them. Next, a considerate portion of respondents thought personal factors such as political views and identities had an influence on prioritizing ethics, a result in line with the results for RQ1. Lastly, the neglect of demographic considerations in feature development suggests that key ethical concerns may be overlooked. 
% \end{minipage}}



% \fbox{
% \begin{minipage}{.9\linewidth}
% \textbf{Answer to RQ3:}
% The majority of respondents (66\%) indicated that they were rarely or never asked to contribute to software they considered unethical. However, 36\% felt unempowered to intervene when ethical issues occurred. Sharing ethical concerns with higher-level co-workers was fairly common, but these concerns did not always influence the final product, with 37\% indicating their perspectives rarely or never affected outcomes. Overall, the findings suggest that a notable portion of practitioners have limited control over mitigating ethical concerns. 
% \end{minipage}}

% \subsection{Practitioners' Perceptions of Software \textbf{(RQ4)} }
% %\textbf{(RQ4)} \textit{What are software practitioners’ personal perceptions of the software platforms they create and the ethical concerns associated with them?}
% %The results from this survey provide insightful data on software practitioners' personal perceptions of the platforms they create and the associated ethical concerns. In response to the overall societal impact of their company's software 
% % This distribution suggests that most practitioners view the software they create as having a largely positive influence on society, although there is a minority that acknowledges potential harm. 

% \begin{figure}
% \includegraphics[width=.65\columnwidth]{figures/rq4.png}
%   \caption{Responses to research questions RQ4.1 through RQ4.3 , with the \textit{Full} sample then stratified by demographic groups, including BIPOC, Global South (nationality and residence), women, individuals with disabilities, and participants with roles other than product owner or project manager. The demographic groups presented were selected based on statistically significant results. The x-axis represents the research sub-questions, while the y-axis shows the percentage distribution of responses across Likert categories.}
%   \label{fig:rq4}
% \end{figure}

% An overwhelming majority considers the overall societal impact of its company's software as positive \textbf{(RQ4.1)}. Of the respondents, 43.78\% (95/217) indicated that they perceive the software as "Mostly beneficial," while 29.95\% (65/217) considered it "Completely beneficial" (see Figure~\ref{fig:rq4}). Only a small percentage found the software neutral (21.66\%) or harmful (4.61\%). Significant differences in perceptions of societal impact were observed among participants based on nationality (Mann-Whitney U test, $U = 5094.5$, $p < 0.05$) and residential background (Mann-Whitney U test, $U = 5548$, $p < 0.001$) \textbf{(RQ4.1)}.

% Similarly, when asked about the impact of the software on individual end-users \textbf{(RQ4.2)}, the majority found the software to be "Mostly beneficial" (42.40\%, 92/217), with a notable portion considering it "Completely beneficial" (30.41\%, 66/217) (see Figure~\ref{fig:rq4}). A small percentage found the software neutral (23.50\%) or slightly harmful (3.69\%). Statistically significant differences in perceptions of the software's impact on end-users were identified based on role (H test, $H=13.17, p < 0.05$), nationality (Mann-Whitney U test, $U = 5154.5$, $p < 0.05$), residential background (Mann-Whitney U test, $U = 5316$, $p < 0.001$), gender (Mann-Whitney U test, $U = 5291$, $p < 0.01$), sex (Kruskal-Wallis test, $H = 9.73$, $p < 0.01$), and ability (Mann-Whitney U test, $U = 233$, $p < 0.01$) \textbf{(RQ4.2)}. Dunn's post hoc tests revealed that software testers were significantly less likely than data scientists ($Z = -3.05$, $p < 0.05$) and project managers ($Z = -3.09$, $p < 0.05$) to perceive the software's impact on individual end-users as beneficial. Additionally, women were significantly more likely than men to report a positive impact of the software on individual end-users ($Z = -2.85$, $p < 0.01$).

% Lastly, when considering the personal impact of the software on themselves \textbf{(RQ4.3)}, most respondents reported it as "Mostly beneficial" (44.44\%, 64/144), with a considerable number finding it "Completely beneficial" (38.89\%, 56/144) (see Figure~\ref{fig:rq4}). Very few found the software neutral (14.58\%) or harmful (2.08\%). Statistically significant differences in perceptions of personal impact were observed based on nationality (Mann-Whitney U test, $U = 2296$, $p < 0.01$), residential background (Mann-Whitney U test, $U = 2439.5$, $p < 0.01$), gender (Mann-Whitney U test, $U = 2412.5$, $p < 0.01$), and sex (Kruskal-Wallis test, $H = 8.30$, $p < 0.05$). Dunn's test further indicated that women were significantly more likely than men to report a positive personal impact from the software ($Z = -2.85$, $p < 0.01$).



%For all survey questions where demographic effects were observed, we identified a total of 293 interactions between demographic characteristics. These interactions underscore the nuanced and multifaceted nature of demographic variables in the context of ethics handling. For instance, while women may generally report ethical issues more frequently, men of lower socioeconomic status may report such issues at a higher rate compared to women of higher socioeconomic status. These interaction effects are summarized in Table~\ref{table:summ_interaction}, with the number of interactions per research question and demographic detailed in the Appendix. A comprehensive list of all interactions is provided in the accompanying replication package.

% \begin{center}
% \fbox{\begin{minipage}{.9\linewidth}
% \textbf{Answer to RQ4:}
% Software practitioners generally perceive the platforms they create as having a positive impact, with only a small minority reporting harm. A statistically significant negative correlation was found between viewing the software as beneficial to society and the presence of ethical issues, suggesting that those recognizing more ethical concerns tend to see less societal benefit. While most practitioners use their company's software, non-usage was primarily due to being outside the target user group, with only a few citing ethical concerns. 
% \end{minipage}}
% \end{center}


==> rebuttal.tex <==
We appreciate the reviewers' insightful feedback and recognize the need to more clearly articulate how our study expands upon prior work. While our research builds on Widder et al. (2023) and Madaio et al. (2020) by identifying disparities in ethics handling within software development, it moves beyond these studies by examining a new population with distinct cultural influences. Widder et al.'s participant pool was predominantly male (70\%, 80/115) and overwhelmingly Western, with 89\% of respondents from North America or Europe~\cite{widder2023s}. The assumption that findings from this demographic apply universally overlooks the reality that ethics integration is deeply shaped by culture. Madaio et al. (who only disclose participants' gender) found that AI fairness efforts are largely driven by individual advocates who encounter sociocultural barriers when raising concerns~\cite{madaio2020co}. However, our findings challenge the assumption that marginalization universally suppresses ethical advocacy. Specifically, Black women from the Global South in our study reported a significantly greater capacity to intervene in ethical decision-making compared to white men from the Global North. To explain this disparity, we introduce Ubuntu philosophy as a crucial framework for understanding ethical participation in software development. The following section outlines this addition to the discussion:

Our findings indicate that marginalized groups report feeling more valued, are more likely to share their perspectives on ethical issues, and have a greater capacity to intervene and influence ethical product development. The most significant difference appears between two main groups: white men from the Global North and Black women from the Global South. The latter group's increased capacity to handle ethical concerns is likely influenced by the substantial representation of South African practitioners within this sample (n = 72). Academic literature widely recognizes Ubuntu as the dominant cultural philosophy in sub-Saharan Africa~\cite{mangaliso2018invoking}. Ubuntu asserts that human identity is fundamentally rooted in community, emphasizing collective moral responsibility to society and the environment. 

Furthermore, research has shown that South Africa follows an inclusive rather than exclusive corporate governance regime~\cite{khomba2013shaping}. Unlike the shareholder-centric, hierarchical models prevalent in the US, South Africa’s corporate governance framework emphasizes broad stakeholder involvement, ensuring that decision-making processes account for not only shareholders but also employees, communities, and other affected parties. This inclusive governance structure aligns with the Ubuntu philosophy, reinforcing collective responsibility and ethical deliberation as integral to professional environments.

Ubuntu shapes organizational culture in multiple ways, influencing communication styles, decision-making processes, and approaches to productivity~\cite{mangaliso2018invoking}. Unlike Western business models that prioritize efficiency and individual accountability, Ubuntu places greater emphasis on oral, face-to-face over written communication. Decision-making is consensus-driven, ensuring that dissenting voices are acknowledged rather than overridden by majority rule. Employees are encouraged to express their perspectives, and while this process can be time-intensive, it is valued for fostering cohesion. Additionally, Ubuntu-oriented work environments prioritize harmonious interpersonal relationships over the maximization of productivity, with social considerations taking precedence over economic imperatives~\cite{mangaliso2018invoking}. This emphasis on collective responsibility fosters a broader sense of accountability, where ethical concerns are addressed through open dialogue rather than unilateral directives. The open communication enhances transparency, ensuring that ethical considerations are collectively acknowledged and  scrutinized rather than obscured by hierarchy.

Whether these alternative business practices lead to more ethical outcomes in software development remains an open question. However, the Ubuntu framework presents a clear alternative to dominant Western governance models and is actively implemented in a multi-billion-dollar economy. Within an Ubuntu approach to ethics, transparency is not merely a technical feature of AI systems but a social duty that fosters communal trust. This contrasts with normative ethical frameworks where transparency in deontological AI is often reduced to explainability algorithms, assuming that once an AI system is interpretable, it is ethically justified. Such an approach overlooks the necessity for AI developers to be accountable for the broader societal impact of these technologies.

A key concern raised by Reviewer #2 was that our study does not engage with FAccT’s core debates on algorithmic decision-making or bias mitigation. While we acknowledge that our work does not focus directly on technical fairness metrics, we argue that it remains relevant to algorithmic governance, particularly in understanding the conditions under which ethical concerns are raised and acted upon. The ability of practitioners to intervene in ethical concerns directly affects bias mitigation. If certain governance structures enable practitioners to voice concerns more effectively, this has direct implications for fairness, accountability, and transparency. Our study shifts the focus from individual moral responsibility to the structural conditions that enable ethical action. This challenges the dominant deontological AI ethics framework, where fairness is often framed as an abstract principle rather than an embedded social practice. Our findings suggest that AI governance should incorporate lessons from Ubuntu-inspired participatory governance models rather than relying solely on top-down regulatory enforcement or corporate AI ethics teams.

Additionally, Elias et al. recently conducted a study with Tjikhoeri et al.’s framework and their findings demonstrate that algorithmic unfairness, particularly in recommendation systems, is intrinsically linked to user manipulation, opaque data collection, and the erosion of fundamental rights, including freedom, privacy, accountability, and transparency. These findings underscore the interconnected nature of ethical concerns, challenging the notion that they can be neatly categorized. This conclusion is grounded in research employing Tjikhoeri et al.’s framework, which has not been explored within the FAccT community. Our use of this framework serves not only to introduce an approach that integrates both abstract principles and concrete user feedback to enhance software accountability to end-users, but also to emphasize that ethical challenges must be addressed collectively.

By incorporating Ubuntu into the discussion, we expand the discourse on ethical AI beyond Western, individualist frameworks and highlight the role of cultural factors in shaping ethics integration. Rather than treating fairness, accountability, and transparency as isolated technical properties, we argue for a more comprehensive approach—one that considers the organizational environments in which ethical deliberation occurs. In doing so, our study provides a novel contribution to the FAccT community by demonstrating that ethical engagement in software development is not merely an individual or moral decision but is deeply embedded in governance structures and cultural norms.



